Categorical Semantics for Functional Reactive Programming with Temporal Recursion and Corecursion

Functional reactive programming (FRP) makes it possible to express temporal aspects of computations in a declarative way. Recently we developed two kinds of categorical models of FRP: abstract process categories (APCs) and concrete process categories (CPCs). Furthermore we showed that APCs generalize CPCs. In this paper, we extend APCs with additional structure. This structure models recursion and corecursion operators that are related to time. We show that the resulting categorical models generalize those CPCs that impose an additional constraint on time scales. This constraint boils down to ruling out $\omega$-supertasks, which are closely related to Zeno's paradox of Achilles and the tortoise.

==> eptcsdata.tex <==
\providecommand{\firstpage}{127}
\providecommand{\publicationstatus}{N.R. Krishnaswami and P.B. Levy (Eds.): \\Mathematically Structured Functional Programming 2014 (MSFP 2014). \\
EPTCS 153, 2014, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.153.9}{10.4204/EPTCS.153.9}}
\pdfoutput=1

